Schema-Guided Culture-Aware Complex Event Simulation with Multi-Agent Role-Play

Complex news events, such as natural disasters and socio-political conflicts, require swift responses from the government and society. Relying on historical events to project the future is insufficient as such events are sparse and do not cover all possible conditions and nuanced situations. Simulation of these complex events can help better prepare and reduce the negative impact. We develop a controllable complex news event simulator guided by both the event schema representing domain knowledge about the scenario and user-provided assumptions representing case-specific conditions. As event dynamics depend on the fine-grained social and cultural context, we further introduce a geo-diverse commonsense and cultural norm-aware knowledge enhancement component. To enhance the coherence of the simulation, apart from the global timeline of events, we take an agent-based approach to simulate the individual character states, plans, and actions. By incorporating the schema and cultural norms, our generated simulations achieve much higher coherence and appropriateness and are received favorably by participants from a humanitarian assistance organization.

==> tables/1_comparison_wNorms.tex <==
\begin{table*}[ht]
    \begin{tabular}{c|p{4cm}|p{6.5cm}}
        \hline
         &  \textbf{w/o Norms} & \textbf{w/ Norms} \\
         \hline 
        \textbf{\small{character profile}} & \small{Li Wei is a 32-year-old marketing executive living in Shanghai. He is known for his outgoing personality and enjoys attending social events and networking gatherings. Li Wei is health-conscious but often finds himself in crowded places due to his job.} & \small{Li Wei is a 32-year-old marketing executive living in Shanghai.  He is known for his outgoing personality and enjoys attending social events and networking gatherings. Li Wei is health-conscious but often finds himself in crowded places due to his job. \textit{\textbf{He is single and lives in a modern high-rise apartment in the bustling Jing'an District of Shanghai. He holds a Master's degree in Business Administration from Fudan University. Originally from a smaller city in Jiangsu province, he moved to Shanghai ten years ago to pursue his career. Economically, Li Wei is well-off, earning a comfortable salary that allows him to indulge in his interests and maintain a cosmopolitan lifestyle. He usually commutes to work primarily by metro, which is efficient and fits his environmentally conscious values. Although culturally rooted in Confucian values, Li Wei is not particularly religious, focusing more on personal and professional growth.}}} \\
        \textbf{\small{per-character event plan}} & CC & DD \\
        \textbf{\small{per-character event description}} & \small{Unwind at Home: Despite the ongoing outbreak in Jakarta, Andi Pratama decided to go for a morning jog in the park, taking extra precautions to avoid crowded areas and maintain personal hygiene.} & \small{Unwind at Home: During a disease outbreak in Jakarta, Andi Pratama, a devout Muslim, performed the \textbf{Tahajjud prayer} at night in his apartment. As the new year began, he prayed earnestly for his community's well-being. In the morning, after performing \textbf{Fajr prayer} at home, Andi Pratama jogged in a nearby park, embracing the \textbf{"gotong royong" spirit} by carefully avoiding crowded areas and keeping distance from others.} \\
    \end{tabular}
    \caption{Comparison of complex event simulation with and without knowledge enhancement from culture-specific social norms.}
    \label{tab:tab1}
\end{table*}
